Dense and Aligned Captions (DAC) Promote Compositional Reasoning in VL Models

Vision and Language (VL) models offer an effective method for aligning representation spaces of images and text, leading to numerous applications such as cross-modal retrieval, visual question answering, captioning, and more. However, the aligned image-text spaces learned by all the popular VL models are still suffering from the so-called `object bias' - their representations behave as `bags of nouns', mostly ignoring or downsizing the attributes, relations, and states of objects described/appearing in texts/images. Although some great attempts at fixing these `compositional reasoning' issues were proposed in the recent literature, the problem is still far from being solved. In this paper, we uncover two factors limiting the VL models' compositional reasoning performance. These two factors are properties of the paired VL dataset used for finetuning and pre-training the VL model: (i) the caption quality, or in other words `image-alignment', of the texts; and (ii) the `density' of the captions in the sense of mentioning all the details appearing on the image. We propose a fine-tuning approach for automatically treating these factors leveraging a standard VL dataset (CC3M). Applied to CLIP, we demonstrate its significant compositional reasoning performance increase of up to $\sim27\%$ over the base model, up to $\sim20\%$ over the strongest baseline, and by $6.7\%$ on average.

==> Tables/ablation_table.tex <==
% \begin{table}[t]
%   \centering
%    \small
%     \begin{tabular}{l|cccc|ccc|cccc}
%             \toprule
%             &&&&&\multicolumn{3}{c|}{VL-Checklist} & \multicolumn{4}{c}{ARO}\\
%             &AC&Neg&Dense&MIL&Object &Attribute&Relation & VG-R & VG-A & COCO	& FLICKR\\
%             \midrule            
%             CLIP&&&& & 81.58\%&	67.60\%&63.05\% & 59.98\% & 63.18\% & 47.9\% & 60.2\% \\


%             \midrule


%             % SVLC (CVPR23) & 85\% & 71.97\% & 68.95\% \\
%             % cc3m cap(from SVLC paper)
%             A&&&&  &80.93\% & 66.28\% & 55.52\% & 50.19\%  & 62.48\%  & 21.03\%  & 28.82\%  \\
%             % cc3m cap + SVLC negs(SVLC)
%             &&\checkmark&&   & 85\% & 71.97\% & 68.95\%  & 80.61\% & 73.03\% & 84.73\% & 91.7\%\\
%             %cc3m cap + cc3m LLM exp (mil)
%             &&&LLM&\checkmark  & 83.54\% & 68.57\% & 58.32\% & 65.49\% &	62.81\% &	38.56\% & 50.84\% \\
%             %cc3m cap + cc3m LLM exp (neg+mil) + SVLC negs
%             &&\checkmark&LLM&\checkmark  & 86.08\% & 72.15\% & 70.48\% &74.8\% &	67.8\% &	84.1\% & 88.3\%\\
            
%             % cc3m captions + cc3m LLM exp + SVLC negs & 86.08\% & 72.15\% & 70.48\% \\
%             \midrule
%             %blip2 cap
%             B&\checkmark&&&  & 84.41\% & 71.03\% & 63.94\%& 67.26\% &	64.76\% &	29.43\% &	40.6\% \\
%             %blip2 cap + LLM blip2 exp (mil)
%             &\checkmark&&LLM&\checkmark   & 85.41\% & 70.32\% & 59.87\%  &72.93\% &	65.7\% &72.5\% &82.24\% \\
%             % blip2 cap + SVLC negs
%             % &\checkmark&\checkmark&&  & 86.99\% & \textbf{77.36\%} & 87.52\%&80.46\%&73.1\%&	94.05\%&\textbf{96.18\%}\\
%             \midrule
           
%             %blip2 cap + SVLC negs + LLM blip2 exp (rand cap)
%             C&\checkmark&\checkmark&LLM&Rand &	87.26\%	&74.25\%	&81.97\% &77.56\% &	73.7\% &	92.42\% &	94.76\%\\
%             %blip2 cap + SVLC negs + LLM blip2 exp (neg + mil bs 2)
%             &\checkmark&\checkmark&LLM&\checkmark  (BS 2)  & 87.14\% & 75.61\% & 86.51\%& 79.44\% &	72.17\% &	93.51\% &	\textbf{95.82\%} \\
%             %blip2 cap + SVLC negs + LLM blip2 exp (neg + mil bs 5)
%             &\checkmark&\checkmark& LLM&\checkmark (BS 5)   & 87.3\% & \textbf{77.27\%} & 86.41\%  &\textbf{81.28\%}& \textbf{73.91\%}	&\textbf{94.47\%}&	95.68\% \\
%             \midrule 
            
%             % blip2 cap + SVLC negs + DenseCap (neg+mil bs 2)
%             D&\checkmark&\checkmark&SAM&\checkmark (BS 2)  & 82.03\% & 67.33\% & 62.71\% & 58.86\% & 62.44\% & 47.6\% &57.5\%\\
%             %blip2 cap + SVLC negs + DenseCap (neg+mil bs 5)
%             &\checkmark&\checkmark&SAM&\checkmark (BS 5)  & 85.29\% & 72.67\% & 86.6\% &77.01\%&	69.2\% &90.17\% &93.16\%\\
%             %blip2 cap + SVLC negs + DenseCap (neg+mil bs 10)
%             &\checkmark&\checkmark&SAM&\checkmark (BS 10)  & \textbf{88.5\%} & 75.83\% & \textbf{89.75\%} &77.16\% & 70.5\%&91.22\%&	93.88\%\\

            
            

%             %             \midrule
%             % combined alpha = 0.1  & 87.44\% & 77.24\% & 86.26\% &81.11\% & 	73.58\% & 	94.4\% & 	96.08\% \\
%             % combined alpha = 0.25 & 87.81\% & 77.15\% & 87.25\% & 80.77\% & 	72.9\% & 	94.0\% & 	96.2\% \\
%             % combined alpha = 0.5  & 88.09\% & 76.58\% & 87.28\% & 78.8\% &	71.96\% &	93.37\% &	95.86\% \\
%             % combined alpha = 0.75 & 88.21\% & 76.28\% & 88.55\% & 77.43\% &	71.12\% &	92.24\% &	94.86\% \\
%             % combined alpha = 0.9 & 88.50\% & 75.84\% & 89.75\% & 77.4\% &	70.73\% & 91.8\% & 94.7\%\\
%     \bottomrule 
%     \end{tabular}
    
%     \caption{training ablations. LLM extensions are 5 at most so mil bs > 5 is not relevant}
%     \label{tab:ablations}
% \end{table}

\begin{table}[t]
  \centering
   \small
    \begin{tabular}{l|cccc|ccc|cccc}
            \toprule
            &&&&&\multicolumn{3}{c|}{VL-Checklist} & \multicolumn{4}{c}{ARO}\\
            &AC&Neg&Dense&MIL&Object &Attribute&Relation & VG-R & VG-A & COCO	& FLICKR\\
            \midrule            
            CLIP&&&& & 81.58\%&	67.60\%&63.05\% & 59.98\% & 63.18\% & 47.9\% & 60.2\% \\


            \midrule


            % SVLC (CVPR23) & 85\% & 71.97\% & 68.95\% \\
            % cc3m cap(from SVLC paper)
            A&&&&  &80.93\% & 66.28\% & 55.52\% & 50.19\%  & 62.48\%  & 21.03\%  & 28.82\%  \\
            % cc3m cap + SVLC negs(SVLC)
            &&\checkmark&&   & 85\% & 71.97\% & 68.95\%  & 80.61\% & 73.03\% & 84.73\% & 91.7\%\\
            %cc3m cap + cc3m LLM exp (mil)
            &&&LLM&\checkmark  & 83.54\% & 68.57\% & 58.32\% & 65.49\% &	62.81\% &	38.56\% & 50.84\% \\
            %cc3m cap + cc3m LLM exp (neg+mil) + SVLC negs
            &&\checkmark&LLM&\checkmark  & 86.08\% & 72.15\% & 70.48\% &74.8\% &	67.8\% &	84.1\% & 88.3\%\\
            
            % cc3m captions + cc3m LLM exp + SVLC negs & 86.08\% & 72.15\% & 70.48\% \\
            \midrule
            %blip2 cap
            B&\checkmark&&&  & 84.41\% & 71.03\% & 63.94\%& 67.26\% &	64.76\% &	29.43\% &	40.6\% \\
            %blip2 cap + LLM blip2 exp (mil)
            &\checkmark&&LLM&\checkmark   & 85.41\% & 70.32\% & 59.87\%  &72.93\% &	65.7\% &72.5\% &82.24\% \\
            % blip2 cap + SVLC negs
            % &\checkmark&\checkmark&&  & 86.99\% & \textbf{77.36\%} & 87.52\%&80.46\%&73.1\%&	94.05\%&\textbf{96.18\%}\\
            \midrule
           
            %blip2 cap + SVLC negs + LLM blip2 exp (rand cap)
            C&\checkmark&\checkmark&LLM&Rand &	87.26\%	&74.25\%	&81.97\% &77.56\% &	73.7\% &	92.42\% &	94.76\%\\
            %blip2 cap + SVLC negs + LLM blip2 exp (neg + mil bs 2)
            &\checkmark&\checkmark&LLM&\checkmark  (BS 2)  & 87.14\% & 75.61\% & 86.51\%& 79.44\% &	72.17\% &	93.51\% &	\textbf{95.82\%} \\
            %blip2 cap + SVLC negs + LLM blip2 exp (neg + mil bs 5)
            &\checkmark&\checkmark& LLM&\checkmark (BS 5)   & 87.3\% & \textbf{77.27\%} & 86.41\%  &\textbf{81.28\%}& \textbf{73.91\%}	&\textbf{94.47\%}&	95.68\% \\
            \midrule 
            
            % blip2 cap + SVLC negs + DenseCap (neg+mil bs 2)
            D&\checkmark&\checkmark&SAM&\checkmark (BS 2)  & 82.03\% & 67.33\% & 62.71\% & 58.86\% & 62.44\% & 47.6\% &57.5\%\\
            %blip2 cap + SVLC negs + DenseCap (neg+mil bs 5)
            &\checkmark&\checkmark&SAM&\checkmark (BS 5)  & 85.29\% & 72.67\% & 86.6\% &77.01\%&	69.2\% &90.17\% &93.16\%\\
            %blip2 cap + SVLC negs + DenseCap (neg+mil bs 10)
            &\checkmark&\checkmark&SAM&\checkmark (BS 10)  & \textbf{88.5\%} & 75.83\% & \textbf{89.75\%} &77.16\% & 70.5\%&91.22\%&	93.88\%\\

            
            

            %             \midrule
            % combined alpha = 0.1  & 87.44\% & 77.24\% & 86.26\% &81.11\% & 	73.58\% & 	94.4\% & 	96.08\% \\
            % combined alpha = 0.25 & 87.81\% & 77.15\% & 87.25\% & 80.77\% & 	72.9\% & 	94.0\% & 	96.2\% \\
            % combined alpha = 0.5  & 88.09\% & 76.58\% & 87.28\% & 78.8\% &	71.96\% &	93.37\% &	95.86\% \\
            % combined alpha = 0.75 & 88.21\% & 76.28\% & 88.55\% & 77.43\% &	71.12\% &	92.24\% &	94.86\% \\
            % combined alpha = 0.9 & 88.50\% & 75.84\% & 89.75\% & 77.4\% &	70.73\% & 91.8\% & 94.7\%\\
    \bottomrule 
    \end{tabular}
    
    \caption{training ablations. LLM extensions are 5 at most so mil bs > 5 is not relevant}
    \label{tab:ablations}
\end{table}

==> Tables/elevator.tex <==
\begin{table*}[ht!]
    \centering
    \footnotesize
    \addtolength{\tabcolsep}{-3.5pt}
    \scalebox{0.96}{
    \begin{tabular}{l|c|cccccccccccccccccccc}
        \toprule
        Model & Score & \rotatebox[origin=l]{90}{Caltech101} & \rotatebox[origin=l]{90}{CIFAR10} & \rotatebox[origin=l]{90}{CIFAR100} & \rotatebox[origin=l]{90}{Country211} & \rotatebox[origin=l]{90}{DTD} & \rotatebox[origin=l]{90}{EuroSat} & \rotatebox[origin=l]{90}{FER2013} & \rotatebox[origin=l]{90}{FGVCAircraft} & \rotatebox[origin=l]{90}{Food101} & \rotatebox[origin=l]{90}{GTSRB} & \rotatebox[origin=l]{90}{HatefulMemes} & \rotatebox[origin=l]{90}{KittiDistance} & \rotatebox[origin=l]{90}{MNIST} & \rotatebox[origin=l]{90}{Flowers102} & \rotatebox[origin=l]{90}{OxfordPets} & \rotatebox[origin=l]{90}{PatchCamelyon} & \rotatebox[origin=l]{90}{SST2} & \rotatebox[origin=l]{90}{RESISC45} & \rotatebox[origin=l]{90}{StanfordCars} & \rotatebox[origin=l]{90}{VOC2007} \\
        \midrule


    % \multicolumn{22}{l}{ \bf{Zero-Shot Adaptation}} \\
    %  CLIP & 56.8 & 87.5 & 89.9 & 65.1 & 17.2 & 44.4 & 45.6 & 42.1 & 19.6 & 84.0 & 32.8 & 56.0 & 29.0 & 48.1 & 66.5 & 87.1 & 60.7 & 58.4 & 60.0 & 59.7 & 82.6 \\
    % Ours & {\bf\cellcolor{emerald!30}59.3} & {\bf\cellcolor{emerald!30}90.7} & {\bf\cellcolor{emerald!30}94.0} & {\bf\cellcolor{emerald!30}73.7} & 17.1 & {\bf\cellcolor{emerald!30}47.6} & {\bf\cellcolor{emerald!30}53.4} & {\bf\cellcolor{emerald!30}46.8} & {\bf\cellcolor{emerald!30}28.1} & 83.0 & 27.2 & 54.8 & 25.2 & {\bf\cellcolor{emerald!30}50.6} & {\bf\cellcolor{emerald!30}74.0} & {\bf\cellcolor{emerald!30}88.3} & 48.1 & 54.5 & 59.7 & {\bf\cellcolor{emerald!30}87.3} & 81.0 \\

    % \midrule
    \multicolumn{22}{l}{ \bf{5-Shot Linear Probe}} \\
     CLIP & 66.2 & 90.2 & 90.2 & 66.1 & {\bf\cellcolor{emerald!30}16.3} & 61.4 & 71.6 & 44.4 & {\bf\cellcolor{emerald!30}28.9} & {\bf\cellcolor{emerald!30}84.3} & 58.6 & 55.8 & {\bf\cellcolor{emerald!30}50.5} & 77.9 & 93.0 & {\bf\cellcolor{emerald!30}87.9} & 54.5 & 58.5 & 79.2 & {\bf\cellcolor{emerald!30}68.7} & 85.0 \\
    \textsc{blip2+neg} & {\bf\cellcolor{emerald!30}66.4} & {\bf\cellcolor{emerald!30}90.3} & 91.1 & {\bf\cellcolor{emerald!30}70.0} & 16.1 & 57.0 & 77.8 & 50.9 & 28.7 & 82.5 & {\bf\cellcolor{emerald!30}62.5} & 55.4 & 36.6 & {\bf\cellcolor{emerald!30}78.1} & 93.0 & 87.0 & {\bf\cellcolor{emerald!30}61.4} & 59.6 & 79.6 & 66.6 & 84.7 \\
    \textsc{blip2+neg+llm} & 64.9 & 89.7 & {\bf\cellcolor{emerald!30}91.4} & 68.0 & 13.8 & {\bf\cellcolor{emerald!30}62.9} & 65.3 & {\bf\cellcolor{emerald!30}51.9} & 28.4 & 81.8 & 60.5 & {\bf\cellcolor{emerald!30}56.1} & 36.8 & 71.1 & 93.1 & 87.0 & 50.0 & {\bf\cellcolor{emerald!30}59.9} & {\bf\cellcolor{emerald!30}79.7} & 64.9 & 86.0 \\
    \textsc{blpi2+neg+SAM} & 64.3 & 89.2 & 90.1 & 69.1 & 14.2 & 56.6 & {\bf\cellcolor{emerald!30}81.2} & 51.4 & 26.1 & 77.3 & 60.9 & 55.5 & 30.6 & 57.9 & 92.9 & 85.2 & 56.7 & 62.4 & 76.8 & 64.5 & {\bf\cellcolor{emerald!30}86.8} \\

      % \textsc{sivangl+cap} & {\bf\cellcolor{emerald!30}66.7} & 89.6 & 90.5 & 65.6 & 15.5 & {\bf\cellcolor{emerald!30}63.1} & 76.5 & 51.4 & 28.5 & 81.6 & {\bf\cellcolor{emerald!30}62.7} & 55.8 & 33.1 & 80.7 & {\bf\cellcolor{emerald!30}93.3} & 87.4 & 63.5 & 62.8 & {\bf\cellcolor{emerald!30}79.9} & 66.6 & 85.1 \\
      % \textsc{help2+cap} & 66.0 & 89.5 & 90.5 & {\bf\cellcolor{emerald!30}69.4} & 15.4 & 57.7 & 65.6 & 50.2 & 28.0 & 75.9 & 62.6 & 56.0 & 32.8 & {\bf\cellcolor{emerald!30}87.3} & 93.3 & 87.3 & {\bf\cellcolor{emerald!30}63.4} & {\bf\cellcolor{emerald!30}63.1} & 79.6 & 65.1 & {\bf\cellcolor{emerald!30}86.9} \\


        % Model & Score & \rotatebox[origin=l]{90}{Caltech101} & \rotatebox[origin=l]{90}{CIFAR10} & \rotatebox[origin=l]{90}{CIFAR100} & \rotatebox[origin=l]{90}{Country211} & \rotatebox[origin=l]{90}{DTD} & \rotatebox[origin=l]{90}{EuroSat} & \rotatebox[origin=l]{90}{FER2013} & \rotatebox[origin=l]{90}{FGVCAircraft} & \rotatebox[origin=l]{90}{Food101} & \rotatebox[origin=l]{90}{GTSRB} & \rotatebox[origin=l]{90}{HatefulMemes} & \rotatebox[origin=l]{90}{KittiDistance} & \rotatebox[origin=l]{90}{MNIST} & \rotatebox[origin=l]{90}{Flowers102} & \rotatebox[origin=l]{90}{OxfordPets} & \rotatebox[origin=l]{90}{PatchCamelyon} & \rotatebox[origin=l]{90}{SST2} & \rotatebox[origin=l]{90}{RESISC45} & \rotatebox[origin=l]{90}{StanfordCars} & \rotatebox[origin=l]{90}{VOC2007} \\

    
    
    \midrule
    \multicolumn{22}{l}{ \bf{10-Shot Linear Probe}} \\
    CLIP & 69.6 & {\bf\cellcolor{emerald!30}92.0} & 88.3 & 70.0 & {\bf\cellcolor{emerald!30}18.7} & 68.1 & 81.8 & {\bf\cellcolor{emerald!30}53.0} & 35.4 & {\bf\cellcolor{emerald!30}84.8} & 66.7 & {\bf\cellcolor{emerald!30}56.7} & {\bf\cellcolor{emerald!30}52.2} & 89.0 & 95.2 & {\bf\cellcolor{emerald!30}89.5} & 50.0 & 58.9 & 82.4 & {\bf\cellcolor{emerald!30}73.6} & 85.2 \\
    \textsc{blip2+neg} & {\bf\cellcolor{emerald!30}70.5} & 91.8 & {\bf\cellcolor{emerald!30}89.4} & 69.9 & 17.0 & {\bf\cellcolor{emerald!30}69.1} & {\bf\cellcolor{emerald!30}85.2} & 51.8 & {\bf\cellcolor{emerald!30}35.5} & 83.3 & {\bf\cellcolor{emerald!30}68.6} & 55.6 & 49.9 & {\bf\cellcolor{emerald!30}90.9} & {\bf\cellcolor{emerald!30}95.4} & 89.0 & {\bf\cellcolor{emerald!30}66.3} & {\bf\cellcolor{emerald!30}62.5} & 82.4 & 72.8 & 84.7 \\
    \textsc{blip2+neg+llm} & 69.2 & 91.7 & 89.1 & {\bf\cellcolor{emerald!30}72.2} & 16.7 & 69.0 & 83.5 & 51.4 & 34.7 & 82.7 & 68.1 & 56.4 & 50.4 & 86.6 & 95.1 & 83.2 & 52.6 & 62.4 & 80.7 & 71.6& 86.2 \\
    \textsc{blip2+neg+SAM} & 69.4 & 91.2 & 87.8 & 71.8 & 16.0 & 68.1 & 80.0 & 55.3 & 34.0 & 81.1 & 68.0 & 55.5 & 48.9 & 89.4 & 95.3 & 88.2 & 56.7 & 62.4 & 81.1 & 70.5 & {\bf\cellcolor{emerald!30}87.0} \\
        



      % \textsc{sivangl+cap} & 66.7 & 89.6 & 90.5 & 65.6 & 15.5 & 63.1 & 76.5 & 51.4 & 28.5 & 81.6 & 62.7 & 55.8 & 33.1 & 80.7 & 93.3 & 87.4 & 63.5 & 62.8 & 79.9 & 66.6 & 85.1 \\
      % \textsc{help2+cap} & 66.0 & 89.5 & 90.5 & {\bf\cellcolor{emerald!30}69.4} & 15.4 & 57.7 & 65.6 & 50.2 & 28.0 & 75.9 & 62.6 & 56.0 & 32.8 & {\bf\cellcolor{emerald!30}87.3} & 93.3 & 87.3 & {\bf\cellcolor{emerald!30}63.4} & {\bf\cellcolor{emerald!30}63.1} & 79.6 & 65.1 & {\bf\cellcolor{emerald!30}86.9} \\




    \midrule
    \multicolumn{22}{l}{ \bf{20-Shot Linear Probe}} \\
    CLIP & 71.9 & 93.1 & 92.1 & 71.7 & {\bf\cellcolor{emerald!30}19.4} & 72.4 & 83.0 & 54.4 & 40.3 & 85.3 & 75.9 & 55.7 & 49.8 & 90.0 & 95.2 & 90.3 & 61.0 & 58.8 & {\bf\cellcolor{emerald!30}85.4} & {\bf\cellcolor{emerald!30}78.2} & 85.8 \\
    \textsc{blip2+neg} & 72.1 & 93.1 & 89.5 & 73.9 & 17.9 & 73.0 & 86.7 & 52.3 & {\bf\cellcolor{emerald!30}41.7} & {\bf\cellcolor{emerald!30}84.0} & 77.2 & 56.1 & 54.9 & 92.7 & {\bf\cellcolor{emerald!30}95.4} & {\bf\cellcolor{emerald!30}89.9} & 56.0 & 59.8 & 84.2 & 77.7 & 86.1 \\
    \textsc{blip2+neg+llm} & {\bf\cellcolor{emerald!30}73.0} & 92.7 & 92.1 & {\bf\cellcolor{emerald!30}74.0} & 17.4 & {\bf\cellcolor{emerald!30}73.2} & 87.1 & {\bf\cellcolor{emerald!30}56.0} & 38.1 & 83.8 & 76.9 & {\bf\cellcolor{emerald!30}56.5} & 54.0 & {\bf\cellcolor{emerald!30}94.6} & 95.1 & 89.1 & 71.3 & 60.0 & 84.5 & 77.0 & 86.8 \\
    \textsc{blpi2+neg+SAM} & 73.0 & 92.0 & 91.4 & 73.6 & 17.0 & 72.3 & {\bf\cellcolor{emerald!30}87.4} & 51.4 & 39.4 & 82.4 & {\bf\cellcolor{emerald!30}77.6} & 56.4 & {\bf\cellcolor{emerald!30}57.4} & 93.7 & 95.3 & 88.5 & {\bf\cellcolor{emerald!30}73.3} & {\bf\cellcolor{emerald!30}60.5} & 85.1 & 76.2 & {\bf\cellcolor{emerald!30}87.5} \\

    
    \midrule
    \multicolumn{22}{l}{ \bf{Full-Shot Linear Probe}} \\
    CLIP & 79.0 & 93.3 & 94.9 & 80.3 & 26.1 & 74.2 & 93.7 & 67.4 & 45.7 & 88.5 & 87.8 & 64.8 & 66.1 & 98.8 & 95.2 & 91.4 & 83.3 & 71.0 & 87.9 & 82.1 & 86.3 \\
    Ours & {\bf\cellcolor{emerald!30}80.1} & {\bf\cellcolor{emerald!30}94.5} & {\bf\cellcolor{emerald!30}96.6} & {\bf\cellcolor{emerald!30}84.1} & 24.2 & {\bf\cellcolor{emerald!30}77.4} & {\bf\cellcolor{emerald!30}95.7} & 66.0 & {\bf\cellcolor{emerald!30}57.1} & 88.0 & 86.4 & 59.7 & {\bf\cellcolor{emerald!30}68.1} & 98.6 & {\bf\cellcolor{emerald!30}98.1} & {\bf\cellcolor{emerald!30}92.5} & {\bf\cellcolor{emerald!30}83.4} & 63.5 & {\bf\cellcolor{emerald!30}89.4} & {\bf\cellcolor{emerald!30}93.1} & 85.0 \\

    %   \textsc{blip2+neg} & 72.1 & 93.1 & 89.5 & 73.9 & 17.9 & 73.0 & 86.7 & 52.3 & 41.7 & 84.0 & 77.2 & 56.1 & 54.9 & 92.7 & 95.4 & 89.9 & 56.0 & 59.8 & 84.2 & 77.7 & 86.1 \\
    % \textsc{blip2+neg+llm} & 73.0 & 92.7 & 92.1 & 74.0 & 17.4 & 73.2 & 87.1 & 56.0 & 38.1 & 83.8 & 76.9 & 56.5 & 54.0 & 94.6 & 95.1 & 89.1 & 71.3 & 60.0 & 84.5 & 77.0 & 86.8 \\
    
    % \textsc{blpi2+neg+SAM} & 73.0 & 89.2 & 90.1 & 69.1 & 14.2 & 56.6 & 81.2 & 51.4 & 26.1 & 77.3 & 60.9 & 55.5 & 30.6 & 57.9 & 92.9 & 85.2 & 56.7 & 62.4 & 76.8 & 64.5 & 86.8 \\
 
    
    \bottomrule
    \end{tabular}
    }
    \addtolength{\tabcolsep}{3.5pt}
    \vspace{3mm}
    \caption{Full-spectrum breakdown results on \textsc{Elevater} using CLIP (ViT-B/32) and 10M retrieved image-text pairs from LAION-400M.
    }
    \label{table:experiment_breakdown}
\end{table*}


% \begin{table*}[ht!]
%     \centering
%     \footnotesize
%     \addtolength{\tabcolsep}{-3.5pt}
%     \scalebox{0.96}{
%     \begin{tabular}{l|c|cccccccccccccccccccc}
%         \toprule
%         Strategy & Score & \rotatebox[origin=l]{90}{Caltech101} & \rotatebox[origin=l]{90}{CIFAR10} & \rotatebox[origin=l]{90}{CIFAR100} & \rotatebox[origin=l]{90}{Country211} & \rotatebox[origin=l]{90}{DTD} & \rotatebox[origin=l]{90}{EuroSat} & \rotatebox[origin=l]{90}{FER2013} & \rotatebox[origin=l]{90}{FGVCAircraft} & \rotatebox[origin=l]{90}{Food101} & \rotatebox[origin=l]{90}{GTSRB} & \rotatebox[origin=l]{90}{HatefulMemes} & \rotatebox[origin=l]{90}{KittiDistance} & \rotatebox[origin=l]{90}{MNIST} & \rotatebox[origin=l]{90}{Flowers102} & \rotatebox[origin=l]{90}{OxfordPets} & \rotatebox[origin=l]{90}{PatchCamelyon} & \rotatebox[origin=l]{90}{SST2} & \rotatebox[origin=l]{90}{RESISC45} & \rotatebox[origin=l]{90}{StanfordCars} & \rotatebox[origin=l]{90}{VOC2007} \\
%         \midrule


%     \multicolumn{22}{l}{ \bf{Zero-Shot Adaptation}} \\
%      & 56.8 & 87.5 & 89.9 & 65.1 & 17.2 & 44.4 & 45.6 & 42.1 & 19.6 & 84.0 & 32.8 & 56.0 & 29.0 & 48.1 & 66.5 & 87.1 & 60.7 & 58.4 & 60.0 & 59.7 & 82.6 \\
%     Locked-Text & {\bf\cellcolor{emerald!30}59.3} & {\bf\cellcolor{emerald!30}90.7} & {\bf\cellcolor{emerald!30}94.0} & {\bf\cellcolor{emerald!30}73.7} & 17.1 & {\bf\cellcolor{emerald!30}47.6} & {\bf\cellcolor{emerald!30}53.4} & {\bf\cellcolor{emerald!30}46.8} & {\bf\cellcolor{emerald!30}28.1} & 83.0 & 27.2 & 54.8 & 25.2 & {\bf\cellcolor{emerald!30}50.6} & {\bf\cellcolor{emerald!30}74.0} & {\bf\cellcolor{emerald!30}88.3} & 48.1 & 54.5 & 59.7 & {\bf\cellcolor{emerald!30}87.3} & 81.0 \\
%     Locked-Text Gated-Image & {\bf\cellcolor{emerald!30}60.7} & {\bf\cellcolor{emerald!30}90.6} & {\bf\cellcolor{emerald!30}91.7} & {\bf\cellcolor{emerald!30}70.7} & {\bf\cellcolor{emerald!30}19.1} & {\bf\cellcolor{emerald!30}49.2} & {\bf\cellcolor{emerald!30}53.8} & {\bf\cellcolor{emerald!30}49.0} & {\bf\cellcolor{emerald!30}30.0} & {\bf\cellcolor{emerald!30}85.1} & 30.5 & 54.1 & 22.2 & {\bf\cellcolor{emerald!30}53.9} & {\bf\cellcolor{emerald!30}76.1} & {\bf\cellcolor{emerald!30}90.1} & 53.9 & {\bf\cellcolor{emerald!30}58.4} & {\bf\cellcolor{emerald!30}62.9} & {\bf\cellcolor{emerald!30}88.9} & {\bf\cellcolor{emerald!30}82.8} \\


%     \midrule
%     \multicolumn{22}{l}{ \bf{Few-Shot Linear Probe}} \\
%      & 65.3 & 89.8 & 90.0 & 67.4 & 17.5 & 59.6 & 73.2 & 47.4 & 28.4 & 84.2 & 52.5 & 56.0 & 44.9 & 71.1 & 90.5 & 88.0 & 63.2 & 57.5 & 76.6 & 65.0 & 84.0 \\
%     Locked-Text & {\bf\cellcolor{emerald!30}69.4} & {\bf\cellcolor{emerald!30}92.2} & {\bf\cellcolor{emerald!30}94.1} & {\bf\cellcolor{emerald!30}76.3} & {\bf\cellcolor{emerald!30}17.6} & {\bf\cellcolor{emerald!30}66.6} & {\bf\cellcolor{emerald!30}82.5} & {\bf\cellcolor{emerald!30}49.9} & {\bf\cellcolor{emerald!30}42.1} & {\bf\cellcolor{emerald!30}84.2} & {\bf\cellcolor{emerald!30}55.0} & 54.9 & 42.2 & {\bf\cellcolor{emerald!30}78.7} & {\bf\cellcolor{emerald!30}96.7} & {\bf\cellcolor{emerald!30}89.0} & 58.5 & 54.2 & {\bf\cellcolor{emerald!30}80.5} & {\bf\cellcolor{emerald!30}89.3} & 83.3 \\
%     Locked-Text Gated-Image & {\bf\cellcolor{emerald!30}68.9} & {\bf\cellcolor{emerald!30}92.5} & {\bf\cellcolor{emerald!30}92.3} & {\bf\cellcolor{emerald!30}71.6} & {\bf\cellcolor{emerald!30}18.9} & {\bf\cellcolor{emerald!30}66.2} & {\bf\cellcolor{emerald!30}74.5} & {\bf\cellcolor{emerald!30}51.8} & {\bf\cellcolor{emerald!30}44.1} & {\bf\cellcolor{emerald!30}85.6} & 51.9 & 54.1 & 42.9 & 68.7 & {\bf\cellcolor{emerald!30}97.0} & {\bf\cellcolor{emerald!30}90.6} & 60.5 & {\bf\cellcolor{emerald!30}60.7} & {\bf\cellcolor{emerald!30}78.8} & {\bf\cellcolor{emerald!30}90.0} & {\bf\cellcolor{emerald!30}84.4} \\
    
    
%     \midrule
%     \multicolumn{22}{l}{ \bf{Few-Shot Full-Model Finetune}} \\
%      & 63.3 & 88.8 & 91.3 & 73.0 & 16.6 & 51.8 & 79.3 & 52.3 & 23.1 & 84.0 & 60.4 & 55.8 & 44.3 & 60.5 & 67.3 & 86.9 & 61.8 & 59.3 & 70.8 & 56.3 & 82.4 \\
%     Locked-Text & {\bf\cellcolor{emerald!30}68.8} & {\bf\cellcolor{emerald!30}93.4} & {\bf\cellcolor{emerald!30}94.2} & {\bf\cellcolor{emerald!30}79.4} & {\bf\cellcolor{emerald!30}16.9} & {\bf\cellcolor{emerald!30}61.2} & 76.0 & 52.2 & {\bf\cellcolor{emerald!30}41.1} & 83.2 & {\bf\cellcolor{emerald!30}77.3} & 54.9 & 44.0 & {\bf\cellcolor{emerald!30}67.5} & {\bf\cellcolor{emerald!30}90.0} & {\bf\cellcolor{emerald!30}88.9} & 57.8 & 53.3 & {\bf\cellcolor{emerald!30}78.0} & {\bf\cellcolor{emerald!30}89.4} & 77.9 \\
%     Locked-Text Gated-Image & {\bf\cellcolor{emerald!30}68.4} & {\bf\cellcolor{emerald!30}91.3} & {\bf\cellcolor{emerald!30}92.2} & {\bf\cellcolor{emerald!30}77.2} & {\bf\cellcolor{emerald!30}18.1} & {\bf\cellcolor{emerald!30}60.1} & {\bf\cellcolor{emerald!30}81.2} & {\bf\cellcolor{emerald!30}52.6} & {\bf\cellcolor{emerald!30}31.8} & {\bf\cellcolor{emerald!30}85.4} & {\bf\cellcolor{emerald!30}69.4} & 54.1 & 40.0 & {\bf\cellcolor{emerald!30}68.3} & {\bf\cellcolor{emerald!30}88.8} & {\bf\cellcolor{emerald!30}89.7} & 61.0 & {\bf\cellcolor{emerald!30}59.9} & {\bf\cellcolor{emerald!30}77.2} & {\bf\cellcolor{emerald!30}87.0} & {\bf\cellcolor{emerald!30}83.3} \\
    
    
%     \midrule
%     \multicolumn{22}{l}{ \bf{Full-Shot Linear Probe}} \\
%      & 78.4 & 86.0 & 95.1 & 79.8 & 25.9 & 75.3 & 93.8 & 67.8 & 44.7 & 88.6 & 86.9 & 63.1 & 65.8 & 98.8 & 94.5 & 91.0 & 83.2 & 71.6 & 88.1 & 82.1 & 86.0 \\
%     Locked-Text & {\bf\cellcolor{emerald!30}80.1} & {\bf\cellcolor{emerald!30}94.5} & {\bf\cellcolor{emerald!30}96.6} & {\bf\cellcolor{emerald!30}84.1} & 24.2 & {\bf\cellcolor{emerald!30}77.4} & {\bf\cellcolor{emerald!30}95.7} & 66.0 & {\bf\cellcolor{emerald!30}57.1} & 88.0 & 86.4 & 59.7 & {\bf\cellcolor{emerald!30}68.1} & 98.6 & {\bf\cellcolor{emerald!30}98.1} & {\bf\cellcolor{emerald!30}92.5} & {\bf\cellcolor{emerald!30}83.4} & 63.5 & {\bf\cellcolor{emerald!30}89.4} & {\bf\cellcolor{emerald!30}93.1} & 85.0 \\
%     Locked-Text Gated-Image & {\bf\cellcolor{emerald!30}80.4} & {\bf\cellcolor{emerald!30}94.5} & {\bf\cellcolor{emerald!30}95.6} & {\bf\cellcolor{emerald!30}81.6} & {\bf\cellcolor{emerald!30}26.3} & {\bf\cellcolor{emerald!30}77.8} & {\bf\cellcolor{emerald!30}95.3} & 67.2 & {\bf\cellcolor{emerald!30}56.5} & {\bf\cellcolor{emerald!30}89.2} & 83.3 & 62.6 & 65.3 & 98.4 & {\bf\cellcolor{emerald!30}98.2} & {\bf\cellcolor{emerald!30}93.6} & {\bf\cellcolor{emerald!30}83.3} & 70.4 & {\bf\cellcolor{emerald!30}89.7} & {\bf\cellcolor{emerald!30}93.5} & {\bf\cellcolor{emerald!30}86.0} \\
    
    
%     \midrule
%     \multicolumn{22}{l}{ \bf{Full-Shot Full-Model Finetune}} \\
%      & 80.3 & 94.0 & 97.8 & 87.0 & 19.1 & 70.1 & 98.1 & 68.9 & 50.7 & 87.7 & 98.6 & 61.9 & 81.0 & 99.5 & 88.5 & 91.6 & 91.0 & 70.6 & 89.4 & 75.8 & 85.7 \\
%     Locked-Text & {\bf\cellcolor{emerald!30}82.2} & {\bf\cellcolor{emerald!30}95.3} & {\bf\cellcolor{emerald!30}98.3} & {\bf\cellcolor{emerald!30}89.0} & {\bf\cellcolor{emerald!30}20.6} & {\bf\cellcolor{emerald!30}75.1} & 98.0 & {\bf\cellcolor{emerald!30}71.6} & {\bf\cellcolor{emerald!30}60.2} & {\bf\cellcolor{emerald!30}88.0} & {\bf\cellcolor{emerald!30}98.7} & 58.1 & 79.2 & {\bf\cellcolor{emerald!30}99.7} & {\bf\cellcolor{emerald!30}95.3} & {\bf\cellcolor{emerald!30}93.4} & 90.4 & 65.1 & {\bf\cellcolor{emerald!30}90.2} & {\bf\cellcolor{emerald!30}92.6} & 85.1 \\
%     Locked-Text Gated-Image & {\bf\cellcolor{emerald!30}81.8} & {\bf\cellcolor{emerald!30}94.6} & {\bf\cellcolor{emerald!30}98.3} & {\bf\cellcolor{emerald!30}87.8} & {\bf\cellcolor{emerald!30}19.5} & {\bf\cellcolor{emerald!30}72.5} & 97.9 & {\bf\cellcolor{emerald!30}70.5} & {\bf\cellcolor{emerald!30}59.7} & {\bf\cellcolor{emerald!30}88.4} & {\bf\cellcolor{emerald!30}98.7} & 58.5 & 73.4 & {\bf\cellcolor{emerald!30}99.6} & {\bf\cellcolor{emerald!30}94.5} & {\bf\cellcolor{emerald!30}93.0} & 89.1 & 70.5 & {\bf\cellcolor{emerald!30}89.7} & {\bf\cellcolor{emerald!30}93.0} & {\bf\cellcolor{emerald!30}86.6} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \addtolength{\tabcolsep}{3.5pt}
%     \vspace{3mm}
%     \caption{Full-spectrum breakdown results on \textsc{Elevater} using CLIP (ViT-B/32) and 10M retrieved image-text pairs from LAION-400M.
%     }
%     \label{table:experiment_breakdown}
% \end{table*}

==> Tables/gradual.tex <==
\begin{table}[b]
  \centering
   \small
    \begin{tabular}{l|ccc|}
            \toprule
            &\multicolumn{3}{c|}{VL-Checklist} \\
            &Object &Attribute&Relation\\
            \midrule 
            cc3m cap(from SVLC paper) &80.93\% & 66.28\% & 55.52\%  \\
            50-50 - BLIP2 cap + cc3m v0 & 82.86\% &	68.2\% &	61.23\% \\
            blip2 cap & 84.41\% & 71.03\% & 63.94\%\\
    \end{tabular}
    \caption{gradual.}
    \label{tab:gradual}
\end{table}

==> Tables/linear_probe.tex <==
\begin{table}
\centering
\begin{tabular}{l|rrll}
                     & \multicolumn{1}{l}{5-shot} & \multicolumn{1}{l}{10-shot} & 20 shot                         & full-shot   \\
                     \midrule
CLIP~\cite{clip}        & 66.19\%                & 69.58\%                 & \multicolumn{1}{r}{71.90\%} & \multicolumn{1}{r}{78.96\%}  \\
% baseline clipneg     & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}      & NA                              & NA                               \\
% baseline svlc cvpr23 & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}      & NA                              & NA                               \\
% ours blip2+neg       & 66.45\%                    & 70.55\%                & \multicolumn{1}{r}{72.18\%}                              & NA                               \\
\clipdacllm{}   & 64.92\%                & 69.20\%                 & \multicolumn{1}{r}{72.98\%} & {77.44\%}                               \\
\clipdacseg{}   & 64.33\%                & 69.41\%                 & \multicolumn{1}{r}{72.92\%} & {79.3\%}       

\end{tabular}

    \caption{Linear probe on ELEVATER (20 datasets)}
    \label{tab:linear_probe}
\end{table}

==> Tables/main_res.tex <==
\begin{table}
  \centering
   \small
    \begin{tabular}{c|ccc|cccc}
            \toprule
            &\multicolumn{3}{c|}{VL-Checklist} & \multicolumn{4}{c}{ARO}\\
            &Object &Attribute&Relation  & VG-R & VG-A & COCO	& FLICKR\\
            \midrule            
            CLIP\cite{clip} & 81.58\%&	67.60\%&63.05\% & 59.98\% & 63.18\% & 47.9\% & 60.2\% \\
            BLIP\cite{blip}&	89.61\%	&\textbf{80.60\%}&	71.67\%& 59\% &	88\% &	32\% &	37\% \\
            BLIP2\cite{blip2} & 84.14\% & 80.12\% & 70.72\% & - &- &-&-\\
            NegClip\cite{aro} & 81.35\% & 72.236\% & 	63.525\% & 81\%& 71\%&86\%&91\%\\
            SVLC (\cite{svlc}) & 85\% & 71.97\% & 68.95\%  & 80.61\% & 73.03\% & 84.73\% & 91.7\%\\
            \midrule
            % blip2 cap 
            % \clipac{} (Ours)& 84.41\% & 71.03\% & 63.94\%  &67.26\%&64.76\%&29.43\%&40.6\%\\
            % blip2 cap+ SVLC negs & 86.99\% & \textbf{77.36\%} & 87.52\%  &80.46\%&73.1\%&	94.05\%&	\textbf{96.18\%}\\
            % blip2 cap+ SVLC negs + LLM blip2 exp(neg+mil) 
            \clipdacllm{} (Ours)& 87.3\% & {77.27\%} & 86.41\%  &\textbf{81.28\%}& \textbf{73.91\%}	&\textbf{94.47\%}&	95.68\% \\
            %blip2 cap + SVLC negs + DenseCap (neg+mil) 
            \clipdacseg{} (Ours)& \textbf{88.5\%} & 75.829\% & \textbf{89.75\%}  &77.16\% & 70.5\%&91.22\%&	93.88\%\\
            Ours combined  & 88.09\% & 76.58\% & 87.28\% & 78.8\% &	71.96\% &	93.37\% &	\textbf{95.86\%} \\
            \bottomrule
    \end{tabular}
    \caption{All of our experiments were done using the CLIP model. The evaluation was performed using VL-Checklist and ARO.}
    \label{tab:main_res}
\end{table}

==> Tables/vl_checklist_divided.tex <==
\begin{table}
\centering
\begin{tabular}{l|rrrrrrr}
                     & \multicolumn{1}{l}{A-Color} & \multicolumn{1}{l}{A-Material} & \multicolumn{1}{l}{A-Size} & \multicolumn{1}{l}{A-State} & \multicolumn{1}{l}{A-Action} & \multicolumn{1}{l}{R-action} & \multicolumn{1}{l}{R-spatial}  \\
                     \midrule
baseline clip        & 69.95\%                     & 69.35\%                        & 70.05\%                    & 61.30\%                     & 67.54\%                      & 72.60\%                      & 54.00\%                        \\
baseline clipneg     & 73.62\%                     & 75.83\%                        & 66.12\%                    & 75.37\%                     & 70.24\%                      & 66.18\%                      & 60.87\%                        \\
baseline svlc cvpr23 & 77.45\%                     & 77.35\%                        & 73.35\%                    & 62.30\%                     & 69.39\%                      & 74.70\%                      & 63.20\%                        \\
ours blip2+neg       & \textbf{83.20\%}                     & 87.60\%                        & \textbf{76.20\%}                    & 67.65\%                     & 72.15\%                      & 85.63\%                      & 89.40\%                        \\
ours blip2+neg+llm   & 82.15\%                     & \textbf{88.85\%}                        & 74.95\%                    & \textbf{68.05\%}                     & 73.07\%                      & \textbf{85.93\%}                      & 86.00\%                        \\
ours blip2+neg+sam   & 79.05\%                     & 86.35\%                        & 74.40\%                    & 65.50\%                     & \textbf{73.85\%}                      & 85.30\%                      & \textbf{94.20\%}                       
\end{tabular}
\end{table}

==> backup/ablations.tex <==
\section{Ablation study}\label{sec:ablations}

In this section we will ablate the different components of the method and point the contribution of each section. Table~\ref{tab:ablations} details the results for multiple configurations, divided into four section. Each section building upon the other and clarifies the importance of a specific component. The top row of Table~\ref{tab:ablations} show the results of the pretrained CLIP model and is the starting point of all other experiments. All experiments were conducted for the same number of epochs on the same dataset. In the following we will discuss each section and the conclusion that arrise from the results. 
\\
\textbf{Section A} explores the effect of both the SVLC negatives, as published in~\cite{svlc} and the their relation to the LLM expansion when using the original CC3M captions without our Aligned Captions (AC) approach. We see that while adding the LLM expansions improves the VL-Checklist results, we see a degradation in ARO evaluation. We believe that since the LLM expansion is done solely on the captions, and in this scenario the noisy captions only become nosier when expanded using an LLM and thus hurts the ARO evaluation.
\\
\include{Tables/ablation_table}
\textbf{Section B} introduces the Aligned Captions and evaluated the contribution of the LLM expansion upon them. Interestingly, we see an opposite effect to that seen in Section A where the ARO evaluation improves significantly but the VL-checklist performance is degraded.
\\
\textbf{Section C} combines the best of both A and B, and here we see improvement in both VL-Checklist and ARO with respect to the previous sections. We also check the MIL strategy where ``Rand" simply chooses a random sentence from the MIL bag and discards the rest. ``BS 2" an ``BS 5" refer to the MIL bag size, 2 and 5 examples, respectively. We see that increased bag size improves the results and allows the method to learn from more expanded data.
\textbf{Section C} deals with the second method of expansion, using over-segmentation. Here we also ablate the MIL bag-size and show that a bag size of 10 examples outperforms the others and sets the highest score on the VL-Checklist task. However, the LLM method is still stronger on the ARO tasks. 
\\
We see from this extensive ablation section that the in order to truly improve compositional understanding, we first need to start with aligned captions and increase the denseness as much as possible. Due to the computational cost of increasing the MIL bag size, we could not technically increase to greater than 10 examples but we believe that with stronger compute power we can see even better results when moving along these lines.

\include{Tables/ablation_table}

\subsection{Aligned Captions using BLIP2 Captioner}
Vision and Language models are trained on a very large, automatically collected, corpora of image-text pairs such as CC3M\cite{cc3m} or LAION400M{\cite{laion}}. One downside to these datasets is the noisy nature of their captions. While the noise is somewhat suppressed due to the sheer amount of data, it has been shown that the models are still negatively affected. In our experiments we show that the compositional aspects are also greatly affected by the noisy nature of the data. Our first method to improve our model's compositional abilities was done solely by generating aligned captions as described in Section~\ref{sec:quality}. Table~\ref{tab:main_res} shows that our simple CLIP training with Aligned Captions (CLIP-AC) improves over the CLIP~\cite{clip} baseline on most tasks but still falls short from methods that explicitly train the model with these compositionality tasks in mind~ \cite{aro, svlc}.


revisit the caption quality paper we looked at a while ago

1. Caption quality
a. LLM expansion: (i) original captions expansion; (ii) blip captions expansion
b. LLM expansion + filtering: (i) filtering using original captions; (ii) filtering using BLIP
c. comparing the quality (image alignment) of original vs blip vs llm vs dense blips (with sam):
(i) using CLIP score - compare histogram of scores (e.g. scores between 0 and 1 and bins of width 0.1) for original cc3m captions (clip score of matching image with its corresponding text) vs same histogram replacing orig caption with blip caption. Can also just compute an average clip score for both cases.
(ii) GPT4 - llava / mini-gpt4 (ambitious, but does not require train)
(iii) extract nouns and compare to a set of gt annotations in a benchmark that has boxes
d. vary the caption quality and show how it affects some metric (eg. vlc average) if we filter the captions set to be higher quality / lower quality - can also do it simply by mixing original and blip captions gradually (replacing some portion of orig captions with blip).
(i) can compare random replacement to lower quality replacement first

2. Caption density
a. ablate SAM usage - the parameters of the masks, more / less detailed - can also go for a hierarchy
(i) try subsampling the density, but keeping the whole image caption
    (i)a. subsample randomly - ablate subsample size 
    sivan: I did- 2 5 10 (mil batch size)
    (i)b. subsample smartly - by proximity to full image caption? by entailment through llm zero-shot? 
    ... removing duplicates? filter by "tf-idf" - analyze the entire set of captions for repeated phrases and eliminate them
(ii) where to do negatives? (i) full image caption only; (ii) segment caption negative; (iii) both
sivan: where to do negatives? (i) full image caption only; (ii) full image caption + segment caption negative
b. achieving density through LLM + BLIP vs SAM + BLIP
sivan: on the LLM u r talking about blip embedding model and on SAM u r talking about the captioner

3. Systemic
a. MIL variants / parameters 
b. Loss weights
c. Negatives on MIL or not
d. average instead of MIL / random choice
e. freezing ablation (maybe)
e. prompt ablation - ???

4. Ambitious experiment - align our clip with Vicuna using llava :-)

CLIP score (cosine similarity) between CC3M images and: 
(i)cc3m original captions 29.1
(ii) blip2 generated captions on CC3M images 32.4

==> backup/intro.tex <==
\section{Introduction}\label{sec:intro}
Recently, with major discoveries in generative language \cite{chatgpt,gpt4,llama,alpaca,vicuna} and vision \cite{stablediffusion,dalle2} modeling, and Vision \& Language (VL) alignment techniques \cite{clip,blip,blip2,gpt4,minigpt4,llava}, we are getting closer than ever to attaining models capable of complete understanding and knowledge of the surrounding world, as well as being capable of acting w.r.t. this knowledge. The 'eyes' of these emerging systems are the VL models that have been shown to exhibit strong performance in different zero-shot applications, such as recognition \cite{clip,vipergpt,maxi,...}, detection \cite{a,b,c}, segmentation \cite{a,b,c}, visual question-answering \cite{a,b,c}, captioning \cite{blip,blip2,...} and many more. However, despite these great advances, the VL models are known to still suffer from significant drawbacks in compositional reasoning - the ability to understand (and properly reflect in the aligned VL representations) the non-object (non-noun) notions appearing on the images and in the text captions, such as object attributes, states, and inter-object relations. This has been publicized and extensively studied in several recent works \cite{vlc,aro,winoground} that also propose metrics for analyzing this phenomenon. This drawback of VL models may lead to undesired biases and misconceptions when combining them with SOTA Large Language Models (LLMs) to build the hallmark of today's AI systems - multi-modal conversational AI. For example, Figure \ref{fig:fig1}a, illustrates a failure mode of Mini-GPT4 \cite{minigpt4}, which successfully aligns one of the most advanced open-source LLMs (Vicuna \cite{vicuna}) with one of the best open-source VL image captioner (BLIP2 \cite{blip2}), demonstrating unprecedented capabilities for multi-modal chat, yet in some cases failing to recognize simple inter-object relations appearing on an image (Fig. \ref{fig:fig1}a) despite successfully recognizing all the objects.

In this work, we offer a simple \oursfull{} (\ours{}) approach to further enhance compositional reasoning abilities of VL models, such as the most popular CLIP \cite{clip}, without sacrificing their zero-shot performance and downstream transferability. On top of the previously proposed techniques of negative text augmentation \cite{svlc,aro}, we further study the effects of automatically improving the 'caption quality' and 'caption density' in a paired VL dataset on the compositional reasoning performance of VL models finetuned on the improved dataset (Fig. \ref{fig:fig1}b). Surprisingly, we find that the low quality of the web-crawled human captions, that fueled the enormous 400M \cite{clip} and 9B \cite{laion} paired image-text collections used to train the most widely used VL models \cite{clip,blip,blip2}, is one of the main reasons behind degraded compositional reasoning ability in these models. The main source of the low quality seems to be in the loose coupling many of the captions in these datasets have with their respective paired image. Such as captions mentioning unrelated facts or human emotions, thus contributing a considerable amount of noise to the text to image representation spaces alignment learned by the VL model. Another aspect we found leading to degraded compositional reasoning performance seems to be in the succinctness and partiality of the web-crawled captions. In the majority of cases, these captions do not describe the paired image in its entirety, but rather mention only a part of the image content, commonly missing object states, relations, and attributes appearing on the image. An intuitive effect of this is that many of the details visible to the model on the image side, are not represented on the text side and hence are being suppressed by the contrastive learning objectives driving the representation spaces alignment, leading to under-representation of those details (attributes, relations and states in particular) in the resulting image and text embedding vectors.

Our proposed approach automatically enhances the quality and density of the text captions in a paired VL dataset by using a combination of an image captioning technique \cite{blip2}, large language models \cite{a,b,c}, and a foundation segmentation model \cite{sam}. In addition, we propose a finetuning approach to best leverage the enhanced VL dataset incorporating Multiple Instance Learning (MIL) losses and a variant of the previous SOTA negative text augmentation compositional reasoning improvement methods \cite{svlc,aro}. Enhancing these aspects we are able to significantly boost the compositional reasoning performance of CLIP \cite{clip}, measured on a variety of VL-checklist \cite{vlc} and ARO \cite{aro} benchmarks, by up to $\sim27\%$ in inter-object relations and by over $6.7\%$ over the highest baselines on average. Moreover, following our proposed VL models improvements we observe only a small decrease in their zero-shot performance, and almost no decrease (even a slight increase) in their linear probing accuracy - arguably the most important metric in light of the recent "linear alignment to LLM" based techniques \cite{minigpt4,llava} successfully leveraging these VL models \cite{blip,clip} in multi-modal chat systems closely mimicking GPT-4 \cite{gpt4}.

To summarize, our contributions are as follows: (i) we propose a \oursfull{} (\ours{}) approach for enhancing a VL model's compositional reasoning performance without sacrificing its zero-shot accuracy and more importantly - linear transferability, via automatically enhancing the caption quality and density of any off-the-shelf paired VL dataset and applying the proposed fine-tuning technique utilizing Multiple Instance Learning and negative text augmentation; (ii) applying our proposed approach to the most popular CLIP and finetuning on CC3M enhanced with our technique, we arrive at \ours{}-CLIP, that demonstrates significantly higher compositional reasoning performance on large-scale VL-checklist \cite{vlc} and ARO \cite{aro} benchmarks (of up to $27\%$ absolute improvement in inter-object relations over base CLIP and over $6.7\%$ average improvement over the strongest baselines); (iii) we offer a detailed analysis and ablations of the different aspects of our proposed approach as well as analyze our key observation regarding the importance of the VL dataset caption quality and density factors for enhancing the compositional reasoning of the VL model; (iv) we will release our code and improved \ours{}-CLIP checkpoints for the benefit of the community upon acceptance.

==> backup/method.tex <==
\section{Method}\label{sec:method}
In this section, we detail our \ours{} approach to enhancing the compositional reasoning performance of VL models (e.g. CLIP \cite{clip}). Our approach admits an arbitrary paired VL dataset (we use CC3M \cite{cc3m} in our experiments), applies automatic (no human in the loop) caption quality (Sec. \ref{sec:quality}) and caption density (Sec. \ref{sec:density}) enhancements, and follows with finetuning the VL model on the resulting enhanced dataset employing negative text augmentation (Sec. \ref{sec:neg}), and the collection of losses (Sec. \ref{sec:losses}) which also include Multiple Instance Learning (MIL) losses (Sec. \ref{sec:mil}) to cope with additional noise introduced by the caption density enhancement step (Sec. \ref{sec:density}).

\subsection{Improving caption quality}\label{sec:quality}
One of the drawbacks of the Internet-collected VL datasets \cite{cc3m,laion} is the loose alignment the captions commonly have to their paired images. This likely stems from the heuristics commonly employed for this coupling, such as using co-location on the sources web-pages etc. Additional factors that impact the caption-to-image alignment, or in other words `caption quality', are the ambiguous nature of the captions (different web-page authors refer to the images in different detail), the human authors intent and creativity, and many others. As noted in previous work \cite{that_paper_that_talks_on_caption_quality}, caption quality may negatively affect VL model transfer to downstream tasks. In this work, we analyze for the first time the direct impact caption quality has on the compositional reasoning performance of the VL models.

We employ a straightforward approach to enhancing the quality of the captions. To increase their alignment to their paired images, we use image captioning to generate text directly conditioned on the image. We use BLIP2 \cite{blip2} captioner, which in turn translates the image into 32 encoded tokens that are transfered to a language model (OPT \cite{opt}) that outputs a sentence describing the content of the image. Sec. \ref{sec:ablations} includes an analysis of the effect of this proposed caption-to-image alignment. In particular, we show that: (i) the CLIP matching score statistics are significantly improved with replacing original captions with BLIP captions, and qualitatively they are a better fit in many cases (Fig. \ref{fig:orig_vs_blip2}); (ii) even enhancing the caption quality alone has a positive impact on the compositional reasoning performance of the model; (iii) \ours{} full approach is significantly outperforming BLIP2 \cite{blip2} in terms of compositional reasoning (by over $6.4\%$ on VL-checklist \cite{vlc} and by $XXX\%$ on ARO), indicating caption quality enhancement alone is insufficient.

\subsection{Improving caption density}\label{sec:density}
Another important drawback of Internet-collected VL datasets is their `partiality' or `lack of density'. Intuitively, most of these captions are not intended by web-page authors to be descriptive of the image but rather serve different purposes. Consequently, in most if not all of the cases, these cpations do not tell the complete story of the image in terms of not metioning every detail and not imparting additional knowledge on related concepts from world knowledge. Below, we propose and explore two orthogonal methods for enhancing the density of the captions.

\noindent\textbf{Large Language Model (LLM) knowledge expansion.} One solution, is using either the original caption, or the higher quality caption produced by an image captioner, or both, and use them as a prompt to a Large Language Model (LLM) effectively tapping on its world knowledge acquired from the trillion(s) of tokens training. In our experiments we used the GPT-J open LLM, instructing it to generate an `LLM world knowledge expansion' from a given caption via "what should I expect to see in an image of {caption}?" prompts. We parsed the resulting text into a collection of individual sentences and employed them in our training via MIL losses (Sec. \ref{sec:mil}) in order to account to the caption noise expected with this kind of LLM expansion (Fig. \ref{fig:expansion}). Indeed, the source caption is the only information provided to the LLM, and some facts are likely to be hallucinated and unrelated to the corresponding image. We provide an analysis of the effects of this way of increasing caption density through LLMs as well as of various related design choices in Sec. \ref{sec:ablations}. Interestingly, LLM knowledge expansion alone has a mixed effect on the compositional reasoning performance, however it is very effective in combination with other proposed techniques.
 
\noindent\textbf{Leveraging semantic over-segmentation.} Additional, more image-grounded way to enhance caption density is to decompose the image into a set of segments with consistent language semantics and caption each segment individually or in connected segment groups. Consequently, we employ SAM \cite{sam} to produce a decomposition of an image into a collection of segments (seeded by a grid of points), we refer to this as `semantic over-segmentation' as SAM applied in this way produces segments generaly respecting semantic boundaries between objects, but commonly over-segments, highlighting object parts and other sub-object regions. We caption each segment using BLIP2 \cite{blip2} resulting in a collection of captions for each image. As it is an over-segmentation, some of the resulting segment captions tend to be noisy (Fig. \ref{fig:expansion}) and we also employ them in our training through MIL (Sec. \ref{sec:mil}). The analysis of the segmentation-based expansion and effects of this way of caption density enhancment on the compositional reasoning performance in general is provided in Sec. \ref{sec:ablations}.

\subsection{Negative text augmentation}\label{sec:neg}
While in the VL datasets, e.g. CC3M \cite{cc3m} and LAION \cite{laion}, each image-text pair constitues a single sample, it was shown in recent works that it is possible to significantly enhance the effectiveness of these samples for teaching compositional reasoning to VL models via simple negative text augmentation \cite{svlc,aro}. Using this approach, every image receives a set of captions, one correctly matching the image (the source caption) and one or several manipulated to be negative text samples via changing words within the caption highlighting the importance different compositional reasoning aspects (attributes, relations, actions, states) to the finetuned model. For our \ours{} approach we also employ this negative text augmentation strategy combining it with the \ours{} captions enhancement principles we outlined in Sec. \ref{sec:quality} and Sec. \ref{sec:density}. Specifically, we explore applying this augmentation both to the BLIP2 captions (Sec. \ref{sec:losses}), as well as to the LLM-expanded and Segmentation-expanded captions by their (proposed here) combination with the MIL training losses (Sec. \ref{sec:mil}). Notably, our \ours{} approach attains significant improvements (e.g. over $12\%$ on VL-checklist \cite{vlc}) in compositional reasoning performance over the recent method that have proposed the negative text augmentation \cite{svlc,aro}, underlining the importance of the \ours{} factors outlined above. The effects of negative text augmentation are further explored in Sec. \ref{sec:ablations}.

\subsection{Avoiding forgetting with Parameter Efficient Fine-Tuning}\label{sec:lora}
In this work we explore fine-tuning a large scale pre-trained VL model (e.g. CLIP \cite{clip}, prettrained on 400M image-text pairs) on an enhanced (as explained above in Sec. \ref{sec:quality} and \ref{sec:density}) relatively smaller scale VL dataset (e.g. CC3M \cite{cc3m} with 3M image-text pairs). Intuitively, naively finetuning on the smaller dataset may incur forgetting of the powerful zero-shot and (linear) transfer capabilities of the base model (CLIP). As this is undesirable, similar to other works \cite{svlc,constructvl}, we employ parameter efficient finetuning, or more specifically LoRA \cite{lora} incorporated into all parameters of both vision and text encoders of the model to finetune the otherwise frozen model. As can be seen in the analysis performed in Sec. \ref{sec:ablations}, this strategy not only significantly reduces zero-shot performance forgetting, but completely eliminates linear transfer performance loss, which is arguably the more important parameter due to the recent successful linear alignment integration of CLIP with leading open LLM enabling open, GPT4-like, multi-modal chat applications \cite{llava,minigpt4}.

\subsection{Training Losses}\label{sec:losses}
A dual-encoder VL model (e.g., CLIP \cite{clip} admits a text \& image pair $(T,I)$ and has two components: (i) an image encoder $e_I = \mathcal{E}_I(I)$; (ii) a text encoder $e_T = \mathcal{E}_T(T)$. The text-to-image similarity score is therefore computed as:
\begin{equation}
    \mathcal{S}(T,I) = \exp\left(\frac{\tau e_T^Te_I}{||e_T||^2||e_I||^2}\right),
\end{equation}
where  $\tau$ is a learned temperature parameter.

\noindent\textbf{Contrastive Loss.} As most contemporary VL models, we employ the contrastive CLIP-loss \cite{clip} as one of our losses for each batch  $\mathcal{B}$.
\begin{equation}\label{eq:contrastive}
    \mathcal{L}_{cont} = \sum_{i}log\left(\frac{{S}(T_i,I_i) } {\sum_{j}{{S}(T_i,I_j)}}\right) +log\left(\frac{{S}(T_i,I_i) } {\sum_{k}{{S}(T_k,I_i)}}\right).
\end{equation}

\noindent\textbf{Negatives Loss.} In addition to utilizing negative text augmentation as part of our proposed MIL losses (Sec. \ref{sec:mil}), we employ the following negatives loss applied to the BLIP2 generated captions $T_i$:
\begin{equation}
\label{eq:neg}
    \mathcal{L}_{neg} = \sum_{i}-log\left(\frac{\mathcal{S}(T_i,I_i)}{\mathcal{S}(T_i,I_i) + \mathcal{S}(T_i^{neg},I_i)}\right).
\end{equation}
where $T_i^{neg}$ is the negative text generated from the caption text $T_i$ according to the technique of \cite{svlc}\footnote{using the code kindly shared by the authors of \cite{svlc}}.

\subsection{Multiple Instance Learning (MIL)}\label{sec:mil}
The MIL setting, relaxes the paired assumption and defines a "bag" of $M$ targets $\left\{y_i^m\right\}_{m=0}^{M}$ such that at least one of the targets (e.g. texts) is a positive match to the sample (e.g. image). This weak annotation aligns perfectly with our automatic annotation framework.
In our approach we employ MIL-NCE \cite{MIL-NCE} loss that was originally proposed for visual representation learning from uncurated videos. We adapt the MIL-NCE loss to fit the clip, contrastive loss as follows :
\begin{equation}
\label{eq:mil-nce}
\mathcal{L}_{NCE} = -\frac{1}{B}\sum_i^B\log\frac{\sum_m \exp(x_i^Ty^m_i/\sigma)}{\sum_{j=1}^B\sum_m\exp(x_i^Ty^m_j/\sigma)}    
\end{equation}
We modify the loss in Eq. \ref{eq:mil-nce} to support negative caption alternatives generated by negative text augmentation applied to the dense-caption variants (LLM expansion, Segmentation expansion) in the following way:
... TBD ...

\subsection{Implementation details}\label{sec:impl}
we are using a CLIP model with VIT B/32 architecture. we use pytorch. we use XXX implementation of BLIP2 with YYY LLM choice. we use ZZZ SAM code. we used OOO LLM. we use X batch size, Y learning rate, Z optimizer, N epochs, ....
Our code isprovided in the supplementary and would be released upon acceptance together with the \ours{}-CLIP checkpoints having compositional reasoning performance enhanced by our approach.

% \subsection{Sivan's draft}
% we are using images from a dataset called CC3M. 
% the BLIP2 captioning model is employed to generate captions for these images.
% we are using a CLIP model with VIT B/32 architecture.
% For the generated captions, a negative caption generation technique called 'SVLC negatives generation' or 'SVLC negs' is applied.
% Additionally, the method focuses on creating dense captions using two approaches. The first approach involves utilizing GPT-J LLM to generate captions by instructing the model to predict "what should I expect to see in an image of {caption}?" These captions are generated based on textual input and world knowledge. Subsequently, it is the responsibility of our method to filter out any unrelated captions.
% The second approach involves using SAM for segmentation and BLIP2 for captioning the segmented regions. While most of the captions in this approach are relevant to the image, some may be of lower quality or noise, particularly for certain segments.
% To incorporate multiple sentences per image, when some of them are not connected to the image, a strategy known as MIL-NCE is employed. we combine this strategy with creating negatives for these sentences using the SVLC method and incorporating them into the negative sentences of the MIL method.

% CLIP score (cosine similarity) between CC3M images and: 
% (i)cc3m original captions 29.1
% (ii) blip2 generated captions on CC3M images 32.4

\begin{figure}[h]
\caption{CC3M images with their old CC3M and new BLIP2 generated captions.(1-4) examples for the superior of BLIP2 captions (5) example for a case the BLIP2 captions misses to describe the image. Our method can handle this case}\label{fig:orig_vs_blip2}
\centering
\includegraphics[width=1.1\textwidth]{figures/clip_score_with_fail.pdf}
\end{figure}

==> backup/results.tex <==
\include{Tables/main_res}

\section{Experimental Results}\label{sec:results}

\subsection{Datasets}
\textbf{Training:} Our method was trained on the Conceptual Captions 3M datatset \cite{cc3m} which is a large set of 3 million image-text pairs automatically crawled from the internet. While the dataset includes captions for the images, we have found that our method for recaptioning the images as described in Section??? greatly improves compositional reasoning. We thus discard the original captions from the datatset. 
\\
\textbf{Evaluation:} We evaluate our method on two benchmarks for compositional reasoning, VL-Checklist and ARO, and another for image classification.
\\
\textbf{VL-Checklist~\cite{vlc}} is a benchmark constructed from three datasets, namely Visual Genome~\cite{vg}, SWiG~\cite{swig}, VAW~\cite{vaw}, and HAKE~\cite{hake}. 
Each image is paired with two captions, a positive and negative caption. The negative caption was constructed by changing one word and thus change the meaning of the sentence. 
The negatives are categorized to changes related to objects, attributes, or relations. Each category is further divided into sub-categories such as size, material, color etc. 
\\
\textbf{ARO~\cite{aro}} is a new benchmark that also aims to evaluate VL models in their compositional abilities and check the models' sensitivity to word order in the sentence. Similarly to VL-Checklist, this dataset includes images and captions which are either positively or negatively related. However, unlike the negative examples in VL-Checklist, where a word was switched, the negative sentences here are created only by re-ordering the words. This reordering significantly changes the semantics of the sentence in aspects like attribution, relations and general word order significance.  The benchmark is built upon images and captions from COCO~\cite{coco}, Flick30K~\cite{flickr}, and Visual Genome~\cite{vg}. 
\\
\textbf{Image Classification} We further evaluated our method on 20 classification dataset using the Linear-Probing classification protocol described in the ELEVATER Image Classification Toolkit~\cite{elevater}. 
The evaluation includes 20 different datasets, including common classification datasets such as CIFAR100~\cite{cifar100}, EuroSat~\cite{eurosat}, and others.



\subsection{\ours{} for Compositionality}

In our work we propose two methods to increase the captions density. 
First we explore the use of LLMs, specifically ???, to expand the caption and generate additional information that is plausible one will find in  a scene described by the caption.
We refer to this method as \clipdacllm{}. The second proposed method is the use of over-segmentation methods and short captions generated from these segments. We refer to this method as \clipdacseg{}. Both these methods increase caption density and add information that was not necessarily available in the original caption. Due to the nature of the data, and that fact that we generate multiple captions per image, both methods employ the MIL approach, similarly to~\cite{feta, milnce} as described in section~\ref{sec:mil}. Additionally both methods include the negative caption generation and losses as described in~\cite{svlc}. Table~\ref{tab:main_res} shows that both our methods are significantly better at on most tasks with gains up to 17\% over current SoTA. In section~\ref{sec:ablations} we dive deeper into our proposed method and show the contribution of each component in the method to the overall result.
\include{Tables/linear_probe}
\subsection{\ours{} for Image Classification}

We further evaluate out method on the ELEVATER~\cite{elevater} image classification benchmark, comprised of 20 different image classification datasets. Table~\ref{tab:linear_probe} presents the results of the Linear Probing (LP) technique for image classification. This evaluation checks the image encoder's representation capacity by adding a single linear classification layer on top of the visual representations and training only that layer. We explore different amounts of training data for LP training, i.e 5-shot, 10-shot, 20-shot, and full training. We see that our method is comparable to the baseline CLIP~\cite{clip} and in some cases show some improvement. These experiments show that our \ours{} training approach did not degrade the classification capabilities of the original network.
